Effective Notification Campaigns on the Web: A Matter of Trust, Framing, and Support

Misconfigurations and outdated software are a major cause of compromised websites and data leaks. Past research has proposed and evaluated sending automated security notifications to the operators of misconfigured websites, but encountered issues with reachability, mistrust, and a perceived lack of importance. In this paper, we seek to understand the determinants of effective notifications. We identify a data protection misconfiguration that affects 12.7 % of the 1.3 million websites we scanned and opens them up to legal liability. Using a subset of 4754 websites, we conduct a multivariate randomized controlled notification experiment, evaluating contact medium, sender, and framing of the message. We also include a link to a public web-based self-service tool that is run by us in disguise and conduct an anonymous survey of the notified website owners (N=477) to understand their perspective. We find that framing a misconfiguration as a problem of legal compliance can increase remediation rates, especially when the notification is sent as a letter from a legal research group, achieving remediation rates of 76.3 % compared to 33.9 % for emails sent by computer science researchers warning about a privacy issue. Across all groups, 56.6 % of notified owners remediated the issue, compared to 9.2 % in the control group. In conclusion, we present factors that lead website owners to trust a notification, show what framing of the notification brings them into action, and how they can be supported in remediating the issue.

==> sections/08-bestpractices.tex <==
\section{Best Practices for Notifications}
These are rough notes that will be expanded into a fuller text once we are satisfied with the list of lessons learned.
\discuss{MM: Is this section even relevant at this point or completely redundant with the discussion? I would also be fine with removing it instead of restating the same facts again in a different form.}

On the design of notifications:
\begin{itemize}
    \item The sender has an effect in our study.
    Surprisingly, even though the motives of the private sender were questioned by recipients, it performed better than a computer science group at a well-known university.
    Distrust in motives may have led to increased fixes for some because they were unsure if this was a precursor to legal action?
    \item Letters can lead to increased trust, but only if the sending institution is known.
    For private individuals, we saw indications that they can actually increase the distrust because of unclear motivations for spending money on such a letter.
    \item Using outside incentives like legal regulation can assist in motivating operators to fix their website.
    However, make it very clear that you are not taking legal action yourself.
    \item While we cannot make any claims about the effect of providing a self-service tool on remediation, providing such a tool was overwhelmingly perceived as helpful and for some recipients increased trust in the message by providing a way to verify the claims.
    Ensure that your tool can also be found by Google, as people may mistrust links.
    \item (Probably one or more takeaways from the tool section missing)
    \item Be aware that crazy people are out there, and you might encounter them in your study.
\end{itemize}

\todo{Determine what to do with the notification best practices, placeholder here}
\subsection{Best Practices for Notification Studies}
\todo{This may not end up in the paper}
\todo{Also mention some anecdotes here}
Organizational matters:
\begin{itemize}
    \item Make sure any tool you distribute can also be found via Google (people mistrust links)
    \item (Be aware of related tools and their potential shortcomings)
    \item Make sure everyone who might get a call or message because of the notifications is aware of what is going on to avoid sending mixed messages.
    \item People will call.
    They will Google you if you don't provide a phone number.
    They will call whenever it damn well pleases them, no matter if you give them timeslots.
    \item They may also offer you money, or send gifts without consulting you first.
    %\item (There are loads more here, but they are probably a different paper or not interesting enough to warrant inclusion)
\end{itemize}

